Supersymmetric Nonlinear O(3) Sigma Model on the Lattice

A supersymmetric extension of the nonlinear O(3) sigma model in two spacetime dimensions is investigated by means of Monte Carlo simulations. We argue that it is impossible to construct a lattice action that implements both the O(3) symmetry as well as at least one supersymmetry exactly at finite lattice spacing. It is shown by explicit calculations that previously proposed discretizations fail to reproduce the exact symmetries of the target manifold in the continuum limit. We provide an alternative lattice action with exact O(3) symmetry and compare two approaches based on different derivative operators. Using the nonlocal SLAC derivative for the quenched model on moderately sized lattices we extract the value {\sigma}(2, u_0) = 1.2604(13) for the step scaling function at u_0 = 1.0595, to be compared with the exact value 1.261210. For the supersymmetric model with SLAC derivative the discrete chiral symmetry is maintained but we encounter strong sign fluctuations, rendering large lattice simulations ineffective. By applying the Wilson prescription, supersymmetry and chiral symmetry are broken explicitly at finite lattice spacing, though there is clear evidence that both are restored in the continuum limit by fine tuning of a single mass parameter.

==> pfaffiansign.tex <==
\section{Sign of the Pfaffian Determinant}


% embed this picture into a parbox to prevent it from being section-kidnapped
\FIGURE{
\parbox{\linewidth}{\center\input{pfaffianOverVolume}}
\caption{\label{fig:sigma:pfaffianSignOverVolume}Average sign of the Pfaffian
over the physical volume in units of the fermionic mass at different lattice
sizes.}}
With the fermionic mass as a scale at hand it is now possible to give
$\vev{\sign \Pf Q}$ over the physical volume $m_\text{F}L$. The results are shown in
Fig.~\ref{fig:sigma:pfaffianSignOverVolume} and imply that for the present
lattice sizes the sign problem worsens when the lattice spacing is refined at
fixed volume $m_\text{F}L$, in contrast to the Wess-Zumino models, where
the sign problem becomes weaker in the continuum limit. This turns out to be a
technical problem making simulations close to continuum limit at fixed physical
volume exceptionally hard, so that the present analysis involving the SLAC
derivative is only based on rather small lattice sizes. As was noted earlier, 
the Wilson derivative formulation does not suffer from such frequent sign
changes due to the explicit breaking of chiral symmetry and allows for a
treatment of much larger lattice volumes, however at the cost of larger lattice
artifacts.

